BLAST: Balanced Sampling Time Series Corpus for Universal Forecasting Models

The advent of universal time series forecasting models has revolutionized zero-shot forecasting across diverse domains, yet the critical role of data diversity in training these models remains underexplored. Existing large-scale time series datasets often suffer from inherent biases and imbalanced distributions, leading to suboptimal model performance and generalization. To address this gap, we introduce BLAST, a novel pre-training corpus designed to enhance data diversity through a balanced sampling strategy. First, BLAST incorporates 321 billion observations from publicly available datasets and employs a comprehensive suite of statistical metrics to characterize time series patterns. Then, to facilitate pattern-oriented sampling, the data is implicitly clustered using grid-based partitioning. Furthermore, by integrating grid sampling and grid mixup techniques, BLAST ensures a balanced and representative coverage of diverse patterns. Experimental results demonstrate that models pre-trained on BLAST achieve state-of-the-art performance with a fraction of the computational resources and training tokens required by existing methods. Our findings highlight the pivotal role of data diversity in improving both training efficiency and model performance for the universal forecasting task.

==> tables/raw_data.tex <==
\begin{table*}[ht]
    \centering
    \caption{Raw datasets of BLAST.}
    \renewcommand\arraystretch{0.912}
    \begin{tabular}{p{6.cm}|c|c|c|c|c}
    \toprule[1.5pt]
        \textbf{Dataset} & \textbf{Min Length} & \textbf{Max Length} & \textbf{Mean Length} & \textbf{\# Channels} & \textbf{\# Observations} \\ \midrule
        Acsf1 & 1460 & 1460 & 1460.0 & 100 & 146000 \\ \hline
        Adiac & 176 & 176 & 176.0 & 390 & 68640 \\ \hline
        Alibaba\_Cluster\_Trace\_2018 & 0 & 1727 & 1620.0 & 116818 & 189305908 \\ \hline
        Arrow\_Head & 251 & 251 & 251.0 & 36 & 9036 \\ \hline
        Articulary\_Word\_Recognition & 144 & 144 & 144.0 & 2475 & 356400 \\ \hline
        Atrial\_Fibrillation & 640 & 640 & 640.0 & 30 & 19200 \\ \hline
        Azure\_Vm\_Traces\_2017 & 96 & 8063 & 5551.0 & 159472 & 885149471 \\ \hline
        Basic\_Motions & 100 & 100 & 100.0 & 240 & 24000 \\ \hline
        Bdg-2 & 8292 & 17543 & 14783.25 & 611 & 9451261 \\ \hline
        Beef & 470 & 470 & 470.0 & 30 & 14100 \\ \hline
        Beetle\_Fly & 512 & 512 & 512.0 & 20 & 10240 \\ \hline
        Beijing\_Air\_Quality & 34625 & 35063 & 35023.0 & 132 & 4550879 \\ \hline
        Beijing\_Subway\_30\_Min & 1564 & 1571 & 1569.0 & 552 & 495375 \\ \hline
        Bird\_Chicken & 512 & 512 & 512.0 & 20 & 10240 \\ \hline
        Bitcoin\_Dataset\_Without\_Missing\_Values & 2659 & 4581 & 4186.0 & 18 & 75364 \\ \hline
        Bme & 128 & 128 & 128.0 & 30 & 3840 \\ \hline
        Borealis & 3527 & 7446 & 5550.0 & 15 & 83254 \\ \hline
        Borg\_Cluster\_Data\_2011 & 122 & 7775 & 3717.0 & 286772 & 1064411962 \\ \hline
        Buildings\_900k & 8745 & 8760 & 8759.0 & 1795256 & 15726442322 \\ \hline
        Bull & 17540 & 17543 & 17542.0 & 41 & 719222 \\ \hline
        Car & 577 & 577 & 577.0 & 60 & 34620 \\ \hline
        Car\_Parts & 12 & 51 & 48.0 & 2674 & 130252 \\ \hline
        Cbf & 128 & 128 & 128.0 & 30 & 3840 \\ \hline
        Cdc\_Fluview\_Ilinet & 0 & 1358 & 746.0 & 375 & 279272 \\ \hline
        Cdc\_Fluview\_Who\_Nrevss & 0 & 1359 & 492.0 & 296 & 145786 \\ \hline
        Character\_Trajectories & 60 & 180 & 120.0 & 4266 & 512042 \\ \hline
        China\_Air\_Quality & 0 & 397334 & 12953.0 & 2622 & 16801947 \\ \hline
        Chinatown & 24 & 24 & 24.0 & 20 & 480 \\ \hline
        Chlorine\_Concentration & 166 & 166 & 166.0 & 467 & 77522 \\ \hline
        Cif\_2016 & 28 & 120 & 98.0 & 72 & 7108 \\ \hline
        Cif\_2016\_12 & 47 & 107 & 99.0 & 57 & 5644 \\ \hline
        Cif\_2016\_6 & 21 & 68 & 41.0 & 15 & 618 \\ \hline
        Cin\_Cecgtorso & 1639 & 1639 & 1639.0 & 40 & 65560 \\ \hline
        Cmip6 & 7299 & 7299 & 7299.0 & 14327808 & 104578670592 \\ \hline
        Cockatoo & 17543 & 17543 & 17543.0 & 1 & 17543 \\ \hline
        Coffee & 286 & 286 & 286.0 & 28 & 8008 \\ \hline
        Computers & 720 & 720 & 720.0 & 250 & 180000 \\ \hline
        Covid19\_Energy & 31911 & 31911 & 31911.0 & 1 & 31911 \\ \hline
        Covid\_Deaths & 212 & 212 & 212.0 & 266 & 56392 \\ \hline
        Covid\_Mobility & 367 & 412 & 409.0 & 362 & 143933 \\ \hline
        Cricket & 300 & 1197 & 524.25 & 1818 & 1126656 \\ \hline
        Crop & 46 & 46 & 46.0 & 7200 & 331200 \\ \hline
        Daphnet & 9599 & 55039 & 21759.0 & 45 & 979155 \\ \hline
        Diatom\_Size\_Reduction & 345 & 345 & 345.0 & 16 & 5520 \\ \hline
        Distal\_Phalanx & 80 & 80 & 80.0 & 1400 & 112000 \\ \hline
        Dodger\_Loop & 215 & 288 & 287.6666666666667 & 118 & 33645 \\ \hline
        Dodgers & 50399 & 50399 & 50399.0 & 1 & 50399 \\ \hline
        Dominick & 201 & 399 & 296.0 & 100014 & 29652492 \\ \hline
        Duck\_Duck\_Geese & 270 & 270 & 270.0 & 67250 & 18157500 \\ \hline
        Earthquakes & 512 & 512 & 512.0 & 322 & 164864 \\ \hline
        Ecg & 227899 & 10828799 & 430321.0 & 53 & 22807047 \\ \hline
        Ecg200 & 96 & 96 & 96.0 & 100 & 9600 \\ \hline
        Ecg5000 & 140 & 140 & 140.0 & 500 & 70000 \\ \hline
        Ecgfive\_Days & 136 & 136 & 136.0 & 23 & 3128 \\ \hline
        Eigen\_Worms & 17984 & 17984 & 17984.0 & 768 & 13811712 \\ \hline
        Elecdemand & 17519 & 17519 & 17519.0 & 1 & 17519 \\
    \bottomrule[1.2pt]
    \end{tabular}
    \label{tab:raw_data}
\end{table*}
\begin{table*}[ht]
    \centering
    \renewcommand\arraystretch{0.912}
    \begin{tabular}{p{6.cm}|c|c|c|c|c}
    \toprule[1.5pt]
        \textbf{Dataset} & \textbf{Min Length} & \textbf{Max Length} & \textbf{Mean Length} & \textbf{\# Channels} & \textbf{\# Observations} \\ \midrule
        Electric\_Devices & 96 & 96 & 96.0 & 8926 & 856896 \\ \hline
        Electricity & 156 & 232272 & 92713.25 & 1017 & 51585382 \\ \hline
        Elf & 21791 & 21791 & 21791.0 & 1 & 21791 \\ \hline
        Eoghorizontal\_Signal & 1250 & 1250 & 1250.0 & 362 & 452500 \\ \hline
        Eogvertical\_Signal & 1250 & 1250 & 1250.0 & 362 & 452500 \\ \hline
        Epilepsy & 206 & 206 & 206.0 & 411 & 84666 \\ \hline
        Era5 & 8735 & 8735 & 8735.0 & 11059200 & 96602112000 \\ \hline
        Ercot & 154872 & 154872 & 154872.0 & 8 & 1238832 \\ \hline
        Ering & 65 & 65 & 65.0 & 120 & 7800 \\ \hline
        Ethanol\_Concentration & 1751 & 1751 & 1751.0 & 783 & 1371033 \\ \hline
        Ethanol\_Level & 1751 & 1751 & 1751.0 & 504 & 882504 \\ \hline
        Exchange\_Rate & 7588 & 7588 & 7588.0 & 8 & 60704 \\ \hline
        Face & 62 & 350 & 168.5 & 848944 & 52693880 \\ \hline
        Favorita & 117 & 1687 & 1402.0 & 111894 & 110622186 \\ \hline
        Fifty\_Words & 270 & 270 & 270.0 & 450 & 121500 \\ \hline
        Finger\_Movements & 50 & 50 & 50.0 & 8848 & 442400 \\ \hline
        Fish & 463 & 463 & 463.0 & 175 & 81025 \\ \hline
        Ford\_A & 500 & 500 & 500.0 & 3601 & 1800500 \\ \hline
        Ford\_B & 500 & 500 & 500.0 & 3636 & 1818000 \\ \hline
        Fred\_Md & 728 & 728 & 728.0 & 107 & 77896 \\ \hline
        Freezer\_Regular\_Train & 301 & 301 & 301.0 & 150 & 45150 \\ \hline
        Freezer\_Small\_Train & 301 & 301 & 301.0 & 28 & 8428 \\ \hline
        Fungi & 201 & 201 & 201.0 & 18 & 3618 \\ \hline
        Genesis & 16219 & 16219 & 16219.0 & 6 & 97314 \\ \hline
        Gesture & 8 & 945 & 276.974358974359 & 5846 & 2103799 \\ \hline
        Gfc12\_Load & 39413 & 39413 & 39413.0 & 20 & 788260 \\ \hline
        Gfc14\_Load & 17519 & 17519 & 17519.0 & 1 & 17519 \\ \hline
        Gfc17\_Load & 17543 & 17543 & 17543.0 & 8 & 140344 \\ \hline
        Ghl & 200000 & 200000 & 200000.0 & 126 & 25200000 \\ \hline
        Godaddy & 40 & 40 & 40.0 & 6270 & 250800 \\ \hline
        Gun\_Point & 150 & 150 & 150.0 & 456 & 68400 \\ \hline
        Ham & 431 & 431 & 431.0 & 109 & 46979 \\ \hline
        Hand\_Movement\_Direction & 400 & 400 & 400.0 & 1600 & 640000 \\ \hline
        Hand\_Outlines & 2709 & 2709 & 2709.0 & 1000 & 2709000 \\ \hline
        Handwriting & 152 & 152 & 152.0 & 450 & 68400 \\ \hline
        Haptics & 1092 & 1092 & 1092.0 & 155 & 169260 \\ \hline
        Heartbeat & 405 & 405 & 405.0 & 12444 & 5039820 \\ \hline
        Herring & 512 & 512 & 512.0 & 64 & 32768 \\ \hline
        Hierarchical\_Sales & 1775 & 1797 & 1795.0 & 118 & 211832 \\ \hline
        Hog & 16567 & 17543 & 17502.0 & 24 & 420056 \\ \hline
        Hospital & 84 & 84 & 84.0 & 767 & 64428 \\ \hline
        House\_Twenty & 2000 & 2000 & 2000.0 & 40 & 80000 \\ \hline
        Hzmetro & 2376 & 2376 & 2376.0 & 160 & 291840 \\ \hline
        Ideal & 392 & 16166 & 5783.0 & 217 & 1254929 \\ \hline
        Inline\_Skate & 1882 & 1882 & 1882.0 & 100 & 188200 \\ \hline
        Insect\_Epgregular\_Train & 601 & 601 & 601.0 & 62 & 37262 \\ \hline
        Insect\_Epgsmall\_Train & 601 & 601 & 601.0 & 17 & 10217 \\ \hline
        Insect\_Wingbeat & 2 & 22 & 6.0 & 5000000 & 33594800 \\ \hline
        Insect\_Wingbeat\_Sound & 256 & 256 & 256.0 & 220 & 56320 \\ \hline
        Iops & 7577 & 149160 & 102118.0 & 58 & 5922855 \\ \hline
        Italy\_Power\_Demand & 24 & 24 & 24.0 & 67 & 1608 \\ \hline
        Japanese\_Vowels & 7 & 26 & 15.0 & 3240 & 51288 \\ \hline
        Kdd2022 & 35278 & 35278 & 35278.0 & 134 & 4677869 \\ \hline
        Kdd21 & 6683 & 899999 & 77414.0 & 250 & 19353516 \\ \hline
        Kdd\_Cup\_2018 & 254 & 10905 & 10554.0 & 270 & 2438652 \\ \hline
        Large\_Kitchen\_Appliances & 720 & 720 & 720.0 & 375 & 270000 \\ \hline
        Largest & 0 & 105407 & 104167.8 & 42333 & 4405382726 \\ \hline
        Lcl & 192 & 17543 & 13372.0 & 713 & 9534519 \\
    \bottomrule[1.2pt]
    \end{tabular}
\end{table*}
\begin{table*}[ht]
    \centering
    \renewcommand\arraystretch{0.912}
    \begin{tabular}{p{6.cm}|c|c|c|c|c}
    \toprule[1.5pt]
        \textbf{Dataset} & \textbf{Min Length} & \textbf{Max Length} & \textbf{Mean Length} & \textbf{\# Channels} & \textbf{\# Observations} \\ \midrule
        Libras & 45 & 45 & 45.0 & 360 & 16200 \\ \hline
        Lightning2 & 637 & 637 & 637.0 & 60 & 38220 \\ \hline
        Lightning7 & 319 & 319 & 319.0 & 70 & 22330 \\ \hline
        London\_Smart\_Meters & 288 & 39648 & 29951.0 & 5560 & 166523410 \\ \hline
        Loop\_Seattle & 105119 & 105119 & 105119.0 & 323 & 33953437 \\ \hline
        Los\_Loop & 33872 & 34271 & 34262.0 & 207 & 7092284 \\ \hline
        Lsst & 36 & 36 & 36.0 & 14754 & 531144 \\ \hline
        M1\_Monthly & 48 & 150 & 90.0 & 617 & 55998 \\ \hline
        M1\_Quarterly & 18 & 114 & 48.0 & 203 & 9944 \\ \hline
        M1\_Yearly & 15 & 58 & 24.0 & 181 & 4515 \\ \hline
        M3\_Monthly & 66 & 144 & 117.0 & 1428 & 167562 \\ \hline
        M3\_Other\_Dataset & 71 & 104 & 76.0 & 174 & 13325 \\ \hline
        M3\_Quarterly & 24 & 72 & 48.0 & 756 & 37004 \\ \hline
        M3\_Yearly\_Dataset & 20 & 47 & 28.0 & 645 & 18319 \\ \hline
        M4\_Daily & 107 & 9933 & 2371.0 & 4227 & 10023836 \\ \hline
        M4\_Hourly & 748 & 1008 & 901.0 & 414 & 373372 \\ \hline
        M4\_Monthly & 60 & 2812 & 234.0 & 48000 & 11246411 \\ \hline
        M4\_Quarterly & 24 & 874 & 100.0 & 24000 & 2406108 \\ \hline
        M4\_Weekly & 93 & 2610 & 1035.0 & 359 & 371579 \\ \hline
        M4\_Yearly & 19 & 841 & 37.0 & 23000 & 858458 \\ \hline
        M5 & 124 & 1969 & 1562.0 & 30490 & 47649940 \\ \hline
        M\_Dense & 17519 & 17519 & 17519.0 & 30 & 525570 \\ \hline
        Mallat & 1024 & 1024 & 1024.0 & 55 & 56320 \\ \hline
        Meat & 448 & 448 & 448.0 & 60 & 26880 \\ \hline
        Medical\_Images & 99 & 99 & 99.0 & 381 & 37719 \\ \hline
        Melbourne\_Pedestrian & 15 & 24 & 23.0 & 1194 & 28574 \\ \hline
        Mexico\_City\_Bikes & 780 & 104449 & 78313.0 & 494 & 38687004 \\ \hline
        Mgab & 99999 & 99999 & 99999.0 & 10 & 999990 \\ \hline
        Middle\_Phalanx & 80 & 80 & 80.0 & 1399 & 111920 \\ \hline
        Mitdb & 649999 & 649999 & 649999.0 & 32 & 20799968 \\ \hline
        Mixed\_Shapes & 1024 & 1024 & 1024.0 & 600 & 614400 \\ \hline
        Mote\_Strain & 84 & 84 & 84.0 & 20 & 1680 \\ \hline
        Motor\_Imagery & 3000 & 3000 & 3000.0 & 17792 & 53376000 \\ \hline
        Nab & 1125 & 22693 & 6300.0 & 58 & 365442 \\ \hline
        Nasa-\_Msl & 438 & 6099 & 2444.0 & 54 & 131992 \\ \hline
        Nasa-\_Smap & 311 & 8639 & 5312.0 & 108 & 573722 \\ \hline
        Natops & 51 & 51 & 51.0 & 4320 & 220320 \\ \hline
        Nn5 & 791 & 791 & 791.0 & 111 & 86124 \\ \hline
        Nn5\_Weekly & 113 & 113 & 113.0 & 111 & 12543 \\ \hline
        Non\_Invasive\_Fetal & 750 & 750 & 750.0 & 3600 & 2700000 \\ \hline
        Occupancy & 2664 & 9751 & 5724.0 & 10 & 57248 \\ \hline
        Oikolab\_Weather & 100056 & 100056 & 100056.0 & 8 & 800448 \\ \hline
        Olive\_Oil & 570 & 570 & 570.0 & 30 & 17100 \\ \hline
        Opportunity & 21190 & 50701 & 31380.0 & 465 & 14591427 \\ \hline
        Osuleaf & 427 & 427 & 427.0 & 200 & 85400 \\ \hline
        Pdb & 17519 & 17519 & 17519.0 & 1 & 17519 \\ \hline
        Pedestrian\_Counts & 576 & 96424 & 47459.0 & 66 & 3132346 \\ \hline
        Pems & 144 & 52127 & 23588.333333333332 & 260118 & 113008881 \\ \hline
        Pen\_Digits & 8 & 8 & 8.0 & 14988 & 119904 \\ \hline
        Phalanges\_Outlines\_Correct & 80 & 80 & 80.0 & 1800 & 144000 \\ \hline
        Phoneme & 1024 & 1024 & 1024.0 & 214 & 219136 \\ \hline
        Phoneme\_Spectra & 217 & 217 & 217.0 & 36465 & 7912905 \\ \hline
        Pig\_Airway\_Pressure & 2000 & 2000 & 2000.0 & 104 & 208000 \\ \hline
        Pig\_Art\_Pressure & 2000 & 2000 & 2000.0 & 104 & 208000 \\ \hline
        Pig\_Cvp & 2000 & 2000 & 2000.0 & 104 & 208000 \\ \hline
        Plaid & 100 & 1344 & 323.0 & 537 & 173858 \\ \hline
        Plane & 144 & 144 & 144.0 & 105 & 15120 \\ \hline
        Power\_Cons & 144 & 144 & 144.0 & 180 & 25920 \\
    \bottomrule[1.2pt]
    \end{tabular}
\end{table*}
\begin{table*}[ht]
    \centering
    \renewcommand\arraystretch{0.912}
    \begin{tabular}{p{6.cm}|c|c|c|c|c}
    \toprule[1.5pt]
        \textbf{Dataset} & \textbf{Min Length} & \textbf{Max Length} & \textbf{Mean Length} & \textbf{\# Channels} & \textbf{\# Observations} \\ \midrule
        Project\_Tycho & 72 & 3797 & 1077.0 & 1258 & 1166524 \\ \hline
        Proximal\_Phalanx & 80 & 80 & 80.0 & 1400 & 112000 \\ \hline
        Racket\_Sports & 30 & 30 & 30.0 & 906 & 27180 \\ \hline
        Refrigeration\_Devices & 720 & 720 & 720.0 & 375 & 270000 \\ \hline
        Residential & 451 & 614879 & 536824.0 & 1512 & 787350860 \\ \hline
        Restaurant & 46 & 477 & 356.0 & 809 & 248776 \\ \hline
        Rideshare & 0 & 541 & 532.0 & 2340 & 751815 \\ \hline
        Rock & 2844 & 2844 & 2844.0 & 20 & 56880 \\ \hline
        Saugeenday & 23741 & 23741 & 23741.0 & 1 & 23741 \\ \hline
        Sceaux & 34222 & 34222 & 34222.0 & 1 & 34222 \\ \hline
        Screen\_Type & 720 & 720 & 720.0 & 375 & 270000 \\ \hline
        Self\_Regulation & 896 & 1152 & 1024.0 & 3008 & 3053568 \\ \hline
        Semg\_Hand\_Gender\_Ch2 & 1500 & 1500 & 1500.0 & 300 & 450000 \\ \hline
        Semg\_Hand\_Movement\_Ch2 & 1500 & 1500 & 1500.0 & 450 & 675000 \\ \hline
        Semg\_Hand\_Subject\_Ch2 & 1500 & 1500 & 1500.0 & 450 & 675000 \\ \hline
        Sensor\_Scope & 20732 & 30492 & 27037.0 & 23 & 621861 \\ \hline
        Shapelet\_Sim & 500 & 500 & 500.0 & 20 & 10000 \\ \hline
        Shapes\_All & 512 & 512 & 512.0 & 600 & 307200 \\ \hline
        Shmetro & 8778 & 8808 & 8806.0 & 576 & 3866859 \\ \hline
        Small\_Kitchen\_Appliances & 720 & 720 & 720.0 & 375 & 270000 \\ \hline
        Smart & 8397 & 26303 & 19140.0 & 5 & 95704 \\ \hline
        Smd & 23686 & 28742 & 25561.0 & 281 & 7182727 \\ \hline
        Smooth\_Subspace & 15 & 15 & 15.0 & 150 & 2250 \\ \hline
        Solar & 52 & 7397222 & 1512742.8 & 10607 & 602909146 \\ \hline
        Sony\_Aiborobot & 65 & 70 & 67.5 & 47 & 3155 \\ \hline
        Spain & 35063 & 35063 & 35063.0 & 1 & 35063 \\ \hline
        Spoken\_Arabic\_Digits & 4 & 93 & 39.0 & 85787 & 3421912 \\ \hline
        Stand\_Walk\_Jump & 2500 & 2500 & 2500.0 & 48 & 120000 \\ \hline
        Star\_Light\_Curves & 1024 & 1024 & 1024.0 & 1000 & 1024000 \\ \hline
        Strawberry & 235 & 235 & 235.0 & 613 & 144055 \\ \hline
        Subseasonal & 16467 & 16469 & 16468.0 & 3448 & 56785110 \\ \hline
        Subseasonal\_Precip & 11299 & 11322 & 11321.0 & 862 & 9758796 \\ \hline
        Sunspot\_Dataset\_Without\_Missing\_Values & 73924 & 73924 & 73924.0 & 1 & 73924 \\ \hline
        Svdb & 230399 & 230399 & 230399.0 & 115 & 26495885 \\ \hline
        Swedish\_Leaf & 128 & 128 & 128.0 & 500 & 64000 \\ \hline
        Symbols & 398 & 398 & 398.0 & 25 & 9950 \\ \hline
        Synthetic\_Control & 60 & 60 & 60.0 & 300 & 18000 \\ \hline
        Sz\_Taxi & 2975 & 2975 & 2975.0 & 156 & 464100 \\ \hline
        Taxi\_1h & 734 & 744 & 739.0 & 2428 & 1794292 \\ \hline
        Taxi\_30min & 1469 & 1488 & 1478.0 & 2428 & 3589798 \\ \hline
        Temperature\_Rain & 710 & 725 & 724.0 & 32072 & 22653363 \\ \hline
        Toe\_Segmentation1 & 277 & 277 & 277.0 & 40 & 11080 \\ \hline
        Toe\_Segmentation2 & 343 & 343 & 343.0 & 36 & 12348 \\ \hline
        Tourism & 11 & 333 & 140.33333333333334 & 1311 & 164581 \\ \hline
        Trace & 275 & 275 & 275.0 & 100 & 27500 \\ \hline
        Traffic & 1 & 17544 & 5293.1 & 482061 & 767029904 \\ \hline
        Training\_Corpus\_Kernel\_Synth\_1m & 1024 & 1024 & 1024.0 & 1000000 & 1024000000 \\ \hline
        Training\_Corpus\_Tsmixup\_10m & 13 & 2048 & 1070.0 & 10000000 & 10362118269 \\ \hline
        Two\_Lead\_Ecg & 82 & 82 & 82.0 & 23 & 1886 \\ \hline
        Two\_Patterns & 128 & 128 & 128.0 & 1000 & 128000 \\ \hline
        Uber\_Tlc\_Daily & 181 & 181 & 181.0 & 262 & 47422 \\ \hline
        Uber\_Tlc\_Hourly & 4344 & 4344 & 4344.0 & 262 & 1138128 \\ \hline
        Umd & 150 & 150 & 150.0 & 36 & 5400 \\ \hline
        Us\_Births\_Dataset & 7305 & 7305 & 7305.0 & 1 & 7305 \\ \hline
        Ushcn\_Daily & 1 & 59281 & 37808.0 & 6090 & 198628457 \\ \hline
        Vehicle\_Trips\_Dataset\_Without\_Missing\_Values & 70 & 243 & 128.0 & 329 & 42382 \\ \hline
        Wafer & 152 & 152 & 152.0 & 1000 & 152000 \\ \hline
        Weather & 1332 & 65981 & 14296.0 & 3010 & 43032000 \\
    \bottomrule[1.2pt]
    \end{tabular}
\end{table*}
\begin{table*}[ht]
    \centering
    \renewcommand\arraystretch{0.912}
    \begin{tabular}{p{6.cm}|c|c|c|c|c}
    \toprule[1.5pt]
        \textbf{Dataset} & \textbf{Min Length} & \textbf{Max Length} & \textbf{Mean Length} & \textbf{\# Channels} & \textbf{\# Observations} \\ \midrule
        Weatherbench & 2087 & 350640 & 307852.625 & 675840 & 82753646592 \\ \hline
        Wiki-rolling\_Nips & 791 & 911 & 851.0 & 47675 & 40571425 \\ \hline
        Wiki\_Daily\_100k & 2741 & 2741 & 2741.0 & 100000 & 274100000 \\ \hline
        Wind\_4\_Seconds\_Dataset & 7397147 & 7397147 & 7397147.0 & 1 & 7397147 \\ \hline
        Wind\_Farms & 71 & 527040 & 172255.66666666666 & 1013 & 174658539 \\ \hline
        Wine & 234 & 234 & 234.0 & 57 & 13338 \\ \hline
        Word\_Synonyms & 270 & 270 & 270.0 & 267 & 72090 \\ \hline
        Worms & 900 & 900 & 900.0 & 181 & 162900 \\ \hline
        Worms\_Two\_Class & 900 & 900 & 900.0 & 181 & 162900 \\ \hline
        Yahoo & 740 & 1679 & 1560.0 & 367 & 572599 \\ \hline
        Yoga & 426 & 426 & 426.0 & 300 & 127800 \\
    \bottomrule[1.2pt]
    \end{tabular}
\end{table*}

